Generators and Relations for 2-Qubit Clifford+T Operators

We give a presentation by generators and relations of the group of Clifford+T operators on two qubits. The proof relies on an application of the Reidemeister-Schreier theorem to an earlier result of Greylyn, and has been formally verified in the proof assistant Agda.

==> eptcsdata.tex <==
\providecommand{\firstpage}{13}
\providecommand{\publicationstatus}{S. Gogioso, M. Hoban (Eds.):\\
Quantum Physics and Logic (QPL) 2022\\
EPTCS 394, 2023, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.394.2}{10.4204/EPTCS.394.2}}

